MGPU-TSM: A Multi-GPU System with Truly Shared Memory

The sizes of GPU applications are rapidly growing. They are exhausting the compute and memory resources of a single GPU, and are demanding the move to multiple GPUs. However, the performance of these applications scales sub-linearly with GPU count because of the overhead of data movement across multiple GPUs. Moreover, a lack of hardware support for coherency exacerbates the problem because a programmer must either replicate the data across GPUs or fetch the remote data using high-overhead off-chip links. To address these problems, we propose a multi-GPU system with truly shared memory (MGPU-TSM), where the main memory is physically shared across all the GPUs. We eliminate remote accesses and avoid data replication using an MGPU-TSM system, which simplifies the memory hierarchy. Our preliminary analysis shows that MGPU-TSM with 4 GPUs performs, on average, 3.9x? better than the current best performing multi-GPU configuration for standard application benchmarks.

==> thermal.tex <==
\subsection{Thermal Feasibility}
\label{sec:arch}

To ensure our MGPU-TSM system is viable, we evaluated the physical design and thermal behavior of the system. We leverage the detailed thermal-aware placement and routing of different components as proposed in~\cite{coskun2018cross}. We evaluate the thermal behavior at the maximum power scenario using Hotspot~\cite{huang2006hotspot}. We assumed a square-shaped chip for the CPU and GPU.

Figure~\ref{fig:Ng3} shows the thermal map resulting from our thermal-aware placement. At the maximum power consumption, our thermal-aware placement results in a maximum temperature of 88.6\textdegree C. Typical systems can tolerate temperature up to 100\textdegree C. Hence, even our thermal-aware placement results in a viable system. Note that in our analysis we do not consider any sophisticated cooling method such as liquid cooling which is becoming common for high power density systems~\cite{fan2018analytical, gullbrand2019liquid, khalaj2017review}. With the application of efficient liquid cooling mechanism, we expect the temperature to be lowered. Hence, we can pack more GPUs or HBMs onto the interposer and increase the throughput density (Flop/{mm}$^2$) of the system.
\ignore{
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{./figure/final_heatmap.pdf}
  \caption{Thermal map for an MGPU-TSM system with 4GPUs, 1 CPU and 4 HBM stacks
  on an interposer (50mm $\times$ 50mm) using 2.5D integration
  technology.}
  \label{fig:heatmap}
  %\vspace{-0.25in}
\end{figure}}
